Improving Joint Speech-Text Representations Without Alignment

The last year has seen astonishing progress in text-prompted image generation premised on the idea of a cross-modal representation space in which the text and image domains are represented jointly. In ASR, this idea has found application as joint speech-text encoders that can scale to the capacities of very large parameter models by being trained on both unpaired speech and text. While these methods show promise, they have required special treatment of the sequence-length mismatch inherent in speech and text, either by up-sampling heuristics or an explicit alignment model. In this work, we offer evidence that joint speech-text encoders naturally achieve consistent representations across modalities by disregarding sequence length, and argue that consistency losses could forgive length differences and simply assume the best alignment. We show that such a loss improves downstream WER in both a large-parameter monolingual and multilingual system.

==> sections/abstract.tex <==
\begin{abstract}
The careful construction of audio representations has become a dominant feature in the design of approaches to many speech tasks.  Increasingly, such approaches have emphasized \say{disentanglement}, where a representation contains only parts of the speech signal relevant to transcription while discarding irrelevant information.  In this paper, we construct a representation learning task based on joint modeling of ASR and TTS, and seek to learn a representation of audio that disentangles that part of the speech signal that is relevant to transcription from that part which is not.  We present empirical evidence that successfully finding such a representation is tied to the randomness inherent in training.  We then make the observation that these desired, disentangled solutions to the optimization problem possess unique statistical properties.  Finally, we show that enforcing these properties during training improves WER by 24.5\% relative on average for our joint modeling task.  These observations motivate a novel approach to learning effective audio representations.
\end{abstract}


